Model order reduction for parametric high dimensional models in the analysis of financial risk

This paper presents a model order reduction (MOR) approach for high dimensional problems in the analysis of financial risk. To understand the financial risks and possible outcomes, we have to perform several thousand simulations of the underlying product. These simulations are expensive and create a need for efficient computational performance. Thus, to tackle this problem, we establish a MOR approach based on a proper orthogonal decomposition (POD) method. The study involves the computations of high dimensional parametric convection-diffusion reaction partial differential equations (PDEs). POD requires to solve the high dimensional model at some parameter values to generate a reduced-order basis. We propose an adaptive greedy sampling technique based on surrogate modeling for the selection of the sample parameter set that is analyzed, implemented, and tested on the industrial data. The results obtained for the numerical example of a floater with cap and floor under the Hull-White model indicate that the MOR approach works well for short-rate models.

==> acronyms.tex <==
% acronyms.tex (optinal)
% COMMANDS
%
% \acresetall	flushes the ’memory’ of the macro \ac (ie all "used" marks flushed)
%
% \ac{label}	singular (first time Full Name + (ACRO) and mark as used)
% \acp{label}	plural (as \ac but makes short and/or long forms into plurals)
%
% \acs{lable}	short (ACRO)
% \acf{lable}	“full acronym” (Full Name + (ACRO))
% \acl{lable}	long (_without_ ACRO)
%
% \acsp{label}	short plural (ACROs)
% \acfp{label}	“full acronym” plural (Full Names + (ACROs))
% \aclp{label}	long plural (_without_ ACRO)
%
% \acrodef{label}[acronym]{written out form}	definition
%		for example \acrodef{etacar}[$\eta$ Car]{Eta Carinae},
%		with the restriction that the label should be simple ASCII


% PACKAGE & OPTIONS
% acronym package must be loaded (in the preamble):
%    \usepackage[option1,option2,etc.]{acronym}
% OPTIONS:
%    footnote		The option footnote makes the full name appear as a
%			footnote.
%    nohyperlinks	If hyperref is loaded, all acronyms will link to their
%			glossary entry. With the option nohyperlinks these
%			linkscan be suppressed.
%    printonlyused	Only list used acronyms
%    withpage		In printonlyused-mode show the page number where
%			each acronym was first used.
%    smaller		Make the acronym appear smaller.
%    dua			The option dua stands for “don’t use acronyms”. It
%			leads to a redefinition of \ac and \acp, making the
%			full name appear all the time and suppressing all
%			acronyms but the explicity requested by \acf or \acfp.
%    nolist		The option nolist stands for “don’t write the list of
%			acronyms”.


%% INCLUSION
%%
\section*{List of Acronyms}
\label{sec:acronyms}

\begin{acronym}[ROMSOC] %width of the longest acronym should be matched here
  \acro{EID}{European Industrial Doctorate}
  \acro{ESR}{Early Stage Researcher}
  \acro{ITN}{Innovative Training Networks}
  \acro{MSCA}{Marie Skłodowska-Curie Actions} 
  \acro{ROMSOC}{Reduced Order Modelling, Simulation and Optimization of Coupled systems}
  \acro{TUB}{Technische Universit\"at Berlin}
  \acro{ITMATI}{Technological Institute of Industrial Mathematics}
  \acro{MathConsult}{MathConsult GmbH}
\end{acronym}
\clearpage

